Promoting Graph Awareness in Linearized Graph-to-Text Generation

Generating text from structured inputs, such as meaning representations or RDF triples, has often involved the use of specialized graph-encoding neural networks. However, recent applications of pretrained transformers to linearizations of graph inputs have yielded state-of-the-art generation results on graph-to-text tasks. Here, we explore the ability of these linearized models to encode local graph structures, in particular their invariance to the graph linearization strategy and their ability to reconstruct corrupted inputs. Our findings motivate solutions to enrich the quality of models' implicit graph encodings via scaffolding. Namely, we use graph-denoising objectives implemented in a multi-task text-to-text framework. We find that these denoising scaffolds lead to substantial improvements in downstream generation in low-resource settings.

==> tables/graph_masking_formatting.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{p{\columnwidth}}
    \toprule
    \textbf{Original linearization:} \texttt{( want :arg0 ( boy ) :arg1  ( go :arg0 boy ) )}\\
    \midrule
    \textbf{in}\texttt{( want <X> ( boy ) :arg1  <Y> go :arg0 boy ) )}\\
    \textbf{out}\texttt{<X> :arg0 <Y> ( <Z>}\\
    \bottomrule          
    \end{tabular}
    \caption{The input--output formatting to mask out graph components, following the masking strategy of \citet{Raffel2019-zl}.}
    \label{tab:graph_masking_formatting}
\end{table}

==> tables/results_shuffled_amr.tex <==

\begin{table}[t]
        \centering
        \resizebox{\columnwidth}{!}{
            \begin{tabular}{l r r r}
                    \toprule
                                                           & \multicolumn{3}{c}{\textit{Training Order}}\\
                     &                 \textbf{Canonical} &  \textbf{Reconfigured} & \textbf{Randomized} \\
                    \midrule
                    \textit{Eval. Order}  & & & \\
                    \textbf{Canonical}    & 43.52  &  43.08 & 40.90 \\
                   \textbf{Reconfigured}  & 33.27  &  41.13 & 40.33 \\
                   \textbf{Randomized}    & 22.89  &  31.00 & 39.80 \\
                    \bottomrule
            \end{tabular}
        }
        \caption{BLEU under different linearizations on the LDC2017T10 development set, using \textsc{T5-large}.}
        \label{tab:results_shuffled:amr}
\end{table}

==> tables/results_shuffled_webnlg.tex <==
\begin{table}[t]
        \centering
        \resizebox{\columnwidth}{!}{
            \begin{tabular}{l r r}
                    \toprule
                                                           & \multicolumn{2}{c}{\textit{Training Order}}\\
                     &                 \textbf{Canonical} &  \textbf{Shuffled} \\
                    \midrule
                    \textit{Eval. Order}  &       &  \\
                    \textbf{Canonical}    & 62.56 / 44.73  & 62.55 / 45.09 \\
                   \textbf{Shuffled}      & 54.00 / 39.23 & 59.40 / 42.35\\
                    \bottomrule
            \end{tabular}
        }
        \caption{BLEU under different linearizations on the WebNLG test / test-unseen sets, using \textsc{T5-base}. \hl{Double-check}}
        \label{tab:results_shuffled:webnlg}
\end{table}
